Forensic Similarity for Digital Images

In this paper we introduce a new digital image forensics approach called forensic similarity, which determines whether two image patches contain the same forensic trace or different forensic traces. One benefit of this approach is that prior knowledge, e.g. training samples, of a forensic trace are not required to make a forensic similarity decision on it in the future. To do this, we propose a two part deep-learning system composed of a CNN-based feature extractor and a three-layer neural network, called the similarity network. This system maps pairs of image patches to a score indicating whether they contain the same or different forensic traces. We evaluated system accuracy of determining whether two image patches were 1) captured by the same or different camera model, 2) manipulated by the same or different editing operation, and 3) manipulated by the same or different manipulation parameter, given a particular editing operation. Experiments demonstrate applicability to a variety of forensic traces, and importantly show efficacy on "unknown" forensic traces that were not used to train the system. Experiments also show that the proposed system significantly improves upon prior art, reducing error rates by more than half. Furthermore, we demonstrated the utility of the forensic similarity approach in two practical applications: forgery detection and localization, and database consistency verification.

==> sections/approach_v1.tex <==
\section{Proposed Approach}
\label{sec:approach}

%We propose a new deep learning architecture and training methodology to decide whether two image patches have the same or different architecture.

%To do this, first a convolutional neural network (CNN) is used to output low dimensional feature vector which encodes high-level forensic information about a single image patch. Pairs of these feature vectors are then used as input to a similarity network, which determines whether two image patches have the same or different forensic signature. This architecture is learned in two distinct phases. First in \textit{Learning Phase A}, the feature extractor CNN is learned on a set of training classes A. Then in \textit{Learning Phase B}, the similarity network is learned on a second set of training classes B.

In this section, we describe our proposed forensic similarity system architecture implementation and associated training procedure. Recent advances in multimedia forensics research have shown that deep learning based approaches, and in particularly convolutional neural networks (CNNs), are powerful for many forensic tasks~\cite{bayar2018mislnet}. In our proposed architecture and training procedure, we build upon successful CNN-based techniques used in multimedia forensics literature, as well as propose a number of innovations that are aimed at extracting robust forensic features from images and accurately determining forensic similarity between two image patches.

\subsection{Architecture}
Our proposed system architecture is designed to take two image patches as input, and then output a decision on whether they contain the same -- or different -- forensic trace. 
At a high level, our proposed architecture contains two distinct parts: fist a \textit{feature extractor} maps an image patch into a low-dimensional feature space that encodes high-level forensic information, and a then \textit{similarity network} maps pairs of these forensic features to a score indicating forensic similarity.
%At a high level, our proposed system architecture 

%our proposed architecture first utilizes a CNN, composed of 5 convolutional blocks and 2 fully connected layers, to extract low-dimensional features from an image patch. We call this CNN the feature extractor. Then, a pair of identical feature extractors are used to extract features from a pair image patches. 


%We use a deep-learning model which is depicted in Fig.~\ref{fig:full_arch}. This model has two distinct parts: 1) a feature extractor which inputs an image patch and outputs a low-dimensional feature vector that encodes high-level forensic information about the input image patch, and 2) a similarity network that maps pairs of feature vectors to a similarity score indicating whether the two image patches have the same or different forensic signature.

\subsubsection{Feature extractor}
\label{sec:approach:ssec:arch:sssec:fextractor}
%In our system 
Here we describe the feature extractor architecture that maps an input image patch to a low dimensional feature space, which encodes high level forensic information about the image patch. This is the mapping described by~\eqref{eq:feature_extractor}. Later, these feature representations are used as input to the similarity network.

Developments in machine learning research has shown that convolutional neural networks (CNNs) can be trained as generic feature extractors. That is, a CNN can be trained for one task, then the deep-layer neuron activations of an image fed forward through the trained network are used as input features for a different task~\cite{donahue2014decaf}. These neuron activations are called `deep features,' and are often extracted from the last fully connected layer of a network. Research has shown that deep features from a CNN trained for image recognition task can be used to perform scene recognition tasks~\cite{zhou2014learning} and remote sensing tasks~\cite{penatti2015deep}.

In multimedia forensics research, it has been shown that deep features based approaches also very powerful for digital image forensics tasks. In particular, it has been shown that deep features from a CNN trained for camera model identification transfer very well to other forensic tasks such manipulation detection~\cite{mayer2018unified}. Furthermore, work in~\cite{bondi2017first} showed that deep-features from a network trained on one set of camera models can be used to train an support vector machine to identify a different set of camera models. Work in~\cite{bayar2018open} showed that deep features from a CNN trained on a set of camera models can be used to determine whether the camera model of the input image model was used in training.

%Capturing forensic traces from a digital image is an inherently different problem than many common tasks that are actively being researched in the computer vision community. [Some brief explanation]. For example, given two images taken by two different cameras of the exact same scene at the exact same time, an image-recognition CNN would ideally have the same feature map representations for both images. That is, for content related tasks, the CNN based feature representations should be invariant to conditions such as source camera model or processing history. However, for a forensics-targeted CNN, these two images ideally have very different feature representations. Given the very different nature of forensics problems, a number of multimedia forensic deep learning methods have been developed to explicitly suppress the content of the image (e.g. edges, blobs, shapes), while encouraging the learning forensically salient features (e.g. noise distributions, pixel-neighborhood relationships). [List and cite a few approaches].

In our approach, we utilize a CNN architecture developed in \cite{bayar2018mislnet} to use as a deep feature extractor. This particular architecture has been shown effective for multiple forensic tasks including both manipulation detection~\cite{bayar2016deep,bayar2018mislnet,bayar2017design} and camera model identification~\cite{bayar2017design,mayer2018unified}.
Briefly, the feature extractor contains 5 convolutional blocks, labeled `conv1' through `conv5' in Fig.~\ref{fig:full_arch}. Each convolutional, with the exception of the first, contain a convolutional layer, batch normalization, activation, and pooling. Following the convolutional blocks are 2 fully connected layers, labeled `fc1' and `fc2,' each with 200 neurons and hyperbolic tangent activation. We use the activated neuron values of the `fc2' layer as features, which corresponds to the mapping \eqref{eq:feature_extractor} with feature dimension $N=200$ corresponding to the number of neurons in `fc2.' Further details of this CNN architecture are found in \cite{bayar2018mislnet}.

Notably in our implementation we alter the CNN architecture in three ways. First, we use full color image patches in RGB as input to the network, instead of just the green color channel used in~\cite{bayar2018mislnet}. Since many important forensic features are expressed in and across different color channels, it is important for the network to learn these feature representations. Second, we relax the constraint imposed on the first convolutional layer in \cite{bayar2018mislnet} which is used to encourage the network to learn prediction error residuals by setting the central kernel value to -1 and normalizing the remaining kernel values to +1. While this constraint is useful for forensics tasks of single channel image patches, it is not immediately translatable to color images. Third, we double the number of convolutional kernel filters in the first convolutional layer from 3 to 6. This is done to increase the expressive power of the network.

The feature extractor architecture is depicted by each of the two identical `Feature Extractor' blocks in Fig.~\ref{fig:full_arch}, which shows the full system architecture. In our proposed system, we use two identical feature extractors to map two input image patches $X_1$ and $X_2$ to a feature space $f(X_1)$ and $f(X_2)$. The deep feature space is of dimension 200, correspoding to the number of neurons in layer `fc2.' This Siamese configuration serves to ensure that the system is symmetric, i.e. that $X_1$ and $X_2$ can be switched with no consequence. Siamese networks have been utilized in other similarity system. It also signficantly reduces the training complexity, as only one set of weights needs to be learned, which is shared between the two feature extractors. This is called hard sharing, meaning that both feature extractors have the exact same weight and bias parameters. %The features $f(X_1)$ and $f(X_2)$ are then used as input to the similarity network described below.


%The first convolutional block, labeled `constr' in Fig.~\ref{fig:full_arch}, consists of 6 convolutional kernels, of size 5x5.

%[Describe the constraint + equation]

%Work in~\cite{??} has shown that this constraint can be removed given sufficient training data. In our implementation, we have a large training corpus and do not use this constraint. However, in implementations where there are limited training samples, the constraint may be required.

%Following the first convolutional layer are four convolutional blocks. Each convolutional block contains a convolutional layer, batch normalization, hyberbolic tangent activation, and finally a pooling layer. Details for each layer are shown in Table~\ref{tab:architecture_params}, and are also described in \cite{bayar2018mislnet}.

%This CNN model corresponds to the `Feature extractor' shown in Fig.~\ref{fig:full_arch}.
%The feature extractor used in this work differs from the implementation used in~\cite{mayer2018similarity} in the following ways: we input full color (RGB) images instead of just the green channel, we relax the prediction filter constraint in the first convolutional layer, and we double the number of 5x5 kernels from 3 to 6 in the first convolutional layer.

%During training of the feature extractor, an additional fully connected set of neurons (no activation), with a softmax are added. This forms a network that performs forensic identification (e.g. camera model identification or manipulation detection). %Which task is targeted depends on the training data, which is described further in Sec.~\ref{sec:approach:ssec:training}. 
%In order to map to a particular forensic class

%As a result, after training, this portion of the network, which we call the feature extractor, inputs an image patch and outputs a feature vector of length 200, which encodes high level forensic information about the image patch. 

 %In \cite{bayar2016deep,bayar2018mislnet} this layer typically has a constraint so that each kernel forms a prediction error filter. However, work in~\cite{??} has shown that this constraint can be removed given sufficient training data. In our setup we assume sufficient training example so that constraint is removed, but 

\subsubsection{Similarity network}
\label{sec:approach:ssec:arch:sssec:similarity}
Here, we describe our proposed neural network architecture that maps a pair of forensic feature vectors $f(X_1)$ and $f(X_2)$ to a similarity score $\in [0,1]$. This mapping is described by~\eqref{eq:similarity_map}. The similarity score indicates whether the pair of image patches $X_1$ and $X_2$ have the same or different forensic signature. We call this proposed neural network the similarity network, and is depicted in the right-hand side of Fig.~\ref{fig:full_arch}. Briefly, the network consists of 3 layers of neurons, which we view as a hierarchical mapping of two input features vectors to successive feature spaces and ultimately an output score indicating forensic similarity. We then compare this score to a threshold to decide whether the two image patches have the same or different forensic signature.  %The last layer of this network consists of a single neuron, which we call the `similarity neuron.' This similarity neuron is active when two image patches have the same forensic signature and inactive otherwise.


The first layer of neurons, labeled by `fcA' in Fig.~\ref{fig:full_arch}, contains 2048 neurons with ReLU activation. This layer serves to map an input feature vector $f(X)$ to a new, intermediate feature space $f_{inter}(X)$. We use two identical `fcA' layers, in Siamese (hard sharing) configuration, to map each of the input vectors $f(X_1)$ and $f(X_2)$ into $f_{inter}(X_1)$ and $f_{inter}(X_2)$. [maybe equation here for fully connected layer, making explicit how the mapping is performed and explaining that the weights are learned]
%First, given two image patches, a feature vector representation is calculated for each image patch using the feature extractor as described above in Sec.~\ref{sec:approach:ssec:arch:sssec:fextractor}. Then, each feature is remapped to a new feature space through the first fully connected layer in the similarity network, labeled by `fcA' in Fig.~\ref{fig:full_arch}, containing 2048 neurons each with ReLU activation. Both of the feature vectors are mapped using the same layer `fcA' to ensure that both feautures are mapped to the same feature space (i.e. it does not matter which image patch is X1 and which is X2). This can alternatively be thought as two fully connected layers in a hard sharing (Siamese) configuration. Siamese networks have been used in other works outside of the forensics community to learn similarity representations such as signature verification~\cite{bromley1994signature}.

%Next, we concatenate the two intermiedate feature vectors $f_{inter}(X_1)$ and $f_{inter}(X_2)$, as well as the elementwise multimpaction of $f_{inter}(X_1)$ and $f_{inter}(X_2)$ to form a combined feature vector. 

Next the second layer of neurons, labeled by `fcB' in Fig.~\ref{fig:full_arch}, contains 64 neurons with ReLU activation. As input to this layer, we provide a vector
\begin{equation}
f_{concat}(X_1,X_2) = \left[\begin{matrix}
f_{inter}(X_1)\\
f_{inter}(X_2)\\
f_{inter}(X_1) \odot f_{inter}(X_2)
\end{matrix}\right],
\end{equation}
where $\odot$ is the element-wise product operation. This layer maps the input vector $f_{concat}(X_1,X_2)$ to a new feature space $f_{sim}(X_1,X_2) \in \mathbb{R}^{64}$ that encodes information about how forensic similarity of patches $X_1$ and $X_2$. Work in~\cite{lee2014speaker} showed that the element-wise product of feature vectors were powerful for speaker recognition tasks in learned systems.

Finally, a single neuron with sigmoid activation maps the similarity vector $f_{sim}(X_1,X_2)$ to a single score. We call this neuron the `similarity neuron,' since it outputs a single score $\in [0,1]$, where a small values indicates the input image patches $X_1$ and $X_2$ have different forensic signatures, and larger values indicate that the input image patches have the same forensic signature. To make a decision, we compare the similarity score to a threshold $\tau$.

The proposed similarity network differers from the implementation in~\cite{mayer2018similarity} in that we increase the number of neurons in `fcA' from 1024 to 2048, and we add to the concatenation vector the elementwise multiplication of $f_{inter}(X_1)$ and $f_{inter}(X_2)$.


%Next, the intermediate feature space is then mapped to a similarity feature space through a fully connected neural layer labeled `fcB' in Fig.~\ref{fig:full_arch}, which has 64 neurons and ReLU activation. This layer has the intermediate feature space from X1, X2, as well as the elementwise multiplication of the the intermediate feature space from X1 and X2. Work in~\cite{lee2014speaker} showed the elementwise multiplication of two feature vectors is a useful strategy for combining audio-signature feature vectors for comparison. We find that this approach is also useful in digital image forensics. Finally, this similarity feature space is mapped to a similarity score through a single comparison neuron with sigmoid activation, depicted as the final layer in Fig.~\ref{fig:full_arch}. [use notation on the figure]



\subsection{Training Methodology}
\label{sec:approach:ssec:training}
The above architecture is trained in two parts called \textit{learning phases}. In Learning Phase A, we train the feature extractor to output a low-dimensional feature vector that encodes high level forensic information about an image patch. In Learning Phase B, we train the similarity network to map pairs of feature vectors, one from each input image patch, to a similarity score indicating whether the two image patches have the same or different forensic signature.

\subsubsection{Learning Phase A}
In Learning Phase A, we train the feature extractor described in Sec~\ref{sec:approach:ssec:arch:sssec:fextractor}. Research in~\cite{mayer2018unified} found that it is important to have a robustly trained feature extractor in deep features based systems. They also found that a feature extractor trained for camera model identifaction is highly transferable to other forensic tasks, such as manipulation detection. For this reason, during Learning Phase A, we train the feature extractor to learn camera model identificaiton features.

To do this, we add an aditional softmax layer to the feature extractor, and train the network using stochastic gradient descent with a cross-entropy loss function on the output of the softmax layer. Training is performed for 30 epochs with an initial learning rate of 0.001, which is halved every three epochs.

For training data, we use 2,000,000 training image patches from collected from 50 different camera models. These camera models are from the Dresden Image Database~\cite{gloe2010dresden}, as well as our own collected database. The camera model used in Learning Phase A shown in `Camera Model Set A' in Table~\ref{tab:camera_models}.
%Training is performed using stochastic gradient descent for 30 epochs. We use an initial learning rate of 0.001 [check this], which is halved every three epochs.

%For a training database, we use 2,000,000 training image patches from collected from 50 different camera models. Even though our forensic similarity may be used to target non-camera-model forensic signatures, work in~\cite{mayer2018unified} has shown that camera model features transfer well to other forensic tasks. Because of this, we use this trained model as a starting point for the feature extractor of the forensic similarity system.

\subsubsection{Learning Phase B}
Here, we describe second step of the forensic similarity system training procedure, called Learning Phase B. In this learning phase, we train the similarity network to learn a forensic similarity mapping for any targeted forensic trace, such as whether two image patches were captured by the same or different camera model, or manipulated by the same or different editing operation. We control which forensic signature is targetted by choice of training data provided during training. 

Notably, during Learning Phase B, we allow the error to back propagate through the feature extractor. This allows the feature extractor to learn better feature representations. This significantly differs from the implementation in~\cite{mayer2018similarity}, which used a frozen feature extractor.

We train the similarity network (and update the feature extractor simultaneously) using stochastic gradient descent for 30 epochs, with an initial learning rate of 0.005 which is halved every three epochs.
The descriptions of training data used in learning Phase B are described in the experimental results section, where we investigate the effectiveness for different forensic signatures.



\subsection{Patch Selection}
Here, we describe a method for patch selection employed during evaluation of the forensic similarity system. Anecdotally, we have found that certain image patches do not perform well for forensic analysis. This is corroborrated by findings in~\cite{guera2018reliability}, where a deep learning system is used to predict how reliable an image patch is for forensic analysis. In this paper, we use a much simpler, entropy based image filter.

We view a forensic trace as an amount of information that is related to the processing history or capturing device of the image. An image patch is a channel that encodes this information, which is then extracted and compared by our forensic similarity system. Consequently, an image patch must have sufficient capacity in order to encode forensic information.

When evaluating image patches, we ensure that they have sufficient capacity to encode a forensic trace by measuring their entropy. Here, entropy $h$ is defined as
%
\begin{equation}
h = -\sum^{255}_{k=0}p_k \ln \left(p_k\right),
\end{equation}
%
where $p_k$ is the probability that a pixel has luminance value $k$ in the image patch. Entropy $h$ is measured in nats. We estimate $p_k$ by measuring the proportion of pixels that have luminance value $k$. We estimate $p_k$ from luminance values instead of pixel values since there are $256^3$ possible pixel values, and as a result we would not get a reliable estimate of pixel-value entropy in small image patches.

When comparing image patches, we ensure that both image patches have entropy between 2.4 and 5.3 nats. We chose these values since 95\% of image patches in our database fall within this range. In the experimental results section, we show the effect of choice of entropy has on forensic similarity accuracy.

Intuitively, the minimum threshold for our patch selection method eliminates flat (e.g. saturated) image pathces, which would appear the same regardless of camera model or processing history. It also removes patches with very high entropy. In these cases, there is very high pixel variation in the scene, and as a result it is likely difficult for the feature extractor to extract the non-content related traces that are critical for forensic similarity.

==> tables/cam_class_list.tex <==
\begin{table}[t]\centering
\small
\begin{tabular}{l l l}
\toprule
\multicolumn{3}{l}{\textbf{Manipulation Detection}, $\mathbb{T}_A =$ } \\
%\textbf{Network:} & \textbf{CNN} & \textbf{ERT} & & \textbf{CNN} \\
Unaltered & Median Filter (5x5) & Gauss. Blur ($\sigma = 1.1$)\\
AWGN ($\sigma = 2$) & Bilinear Interp. (x1.5) & JPEG (Q=70) \\
\midrule
\multicolumn{3}{l}{\textbf{Camera Model Identification}, $\mathbb{T}_B =$} \\
Apple iPhone 4s$^*$  &  Nikon Coolpix S710$^\dagger$ &  Rollei RCP-S7325XS$^\dagger$ \\
Apple iPhone 6$^*$ & Nikon D200$^\dagger$ &  Samsung Gal. Note4$^*$  \\
Canon Ixus70$^\dagger$  & Olympus mju-1050SW$^\dagger$ & Samsung Gal. S4$^*$ \\
Casio EX-Z150$^\dagger$ & Panasonic DMC-FZ50$^\dagger$ & Samsung LZ74 wide$^\dagger$ \\
FujiFilm FinePixJ50$^\dagger$ & Pentax OptioA40$^\dagger$ & Samsung NV15$^\dagger$ \\
Kodak M1063$^\dagger$ & Praktica DCZ5.9$^\dagger$ &  Sony DSC-T77$^\dagger$\\
LG Nexus 5x$^*$ & Ricoh GX100$^\dagger$ & \\
\midrule
\multicolumn{3}{l}{\textbf{Limited Training Data Camera Model Identification}, $\mathbb{T}_C =$} \\
HTC One M7$^*$  &  Nikon D70$^\dagger$ &  Sony DSC-W170$^\dagger$ \\
Mot. Droid Maxx$^*$ & Samsung Galaxy S2$^*$ &  \\
\bottomrule
\end{tabular}
\caption{Classes for the three investigated tasks. \\
{\footnotesize Camera models from our database$^*$, and from the Dresden Image Database$^\dagger$}}
\label{tab:classes}
\vspace{-0.75cm}
\end{table}


==> tables/patch_jpeg_result.tex <==
%\begin{table*}[t]\centering
%\caption{Accuracy of camera model comparison with different patch types. Patch pairs from 25 camera models (10 known, 15 unknown)}
%\small 
%\begin{tabular}{l l c c c c c c} 
%\toprule
%&  &\multicolumn{2}{c}{\textit{known + known}} & \textit{unknown + known} & \multicolumn{2}{c}{\textit{unknown + unknown}} & \textit{total}\\
%Patch size &  Compression & same & different & different & same & different & \\
%\midrule
%256x256 & None &  97.38\% & 94.47\% & 93.72\% & 92.82\% & 92.00\% & 94.00\%\\
%128x128 & None & 96.41\% & 93.82\% & 91.51\% & 92.54\% & 89.18\% & 92.64\%\\
%256x256 & JPEG QF=95 &  96.76\% & 91.23\% & 91.22\% & 89.49\% & 90.87\% & 91.83\%\\
%128x128 & JPEG QF=95 &  92.84\% & 88.27\% & 87.64\% & 87.90\% & 86.63\% & 88.63\%\\
%\bottomrule
%\end{tabular}
%\end{table*}

\begin{table}[t]\centering
\caption{Accuracy of camera model comparison on different patch types. Patch pairs from 10 known ($K$), 15 unknown ($U$) camera models. With or without second JPEG compression QF=95.}
\label{tab:patch_jpeg_result}
\begin{tabular}{l l c c c c} 
\toprule
Patch size &  JPEG & $K, K$ & $K,U$ & $U,U$ & Total \\
\midrule
256$\times$256 & None &  95.19\% & 93.27\% & 92.22\% & 93.61\%\\
128$\times$128 & None &  94.54\% & 91.22\% & 90.07\% & 92.02\%\\
256$\times$256 & QF=95 &  94.00\% & 91.22\% & 90.15\% & 91.83\%\\
128$\times$128 & QF=95 &  90.55\% & 87.64\% & 87.37\% & 88.63\%\\
\bottomrule
\end{tabular}
%\vspace{-0.5cm}
\vspace{-4mm}
\end{table}


==> tables/testfile.tex <==
\begin{table*}[t]\centering
\vspace{-4mm}
\caption{Camera models used in training (sets A and B) and testing (set C). Note that $A\cap B =  A\cap C = B\cap C = \emptyset$. \newline $^*$Denotes from the Dresden Image Database~\cite{gloe2010dresden}\vspace{-2.5mm}}
\label{tab:camera_models}
\setlength{\tabcolsep}{0.5em}
\scriptsize
\begin{tabular}{l l l l l l} 
\toprule
\multicolumn{6}{l}{\textbf{{Camera model set A}}} \\ 
Apple iPhone 4& Canon PC1730& Huawei Honor 5x& Nikon Coolpix S7000& Praktica DCZ5.9$^*$& Sony DSC-W800\\ 
Apple iPhone 4s& Canon Powershot A580& LG G2& Nikon Coolpix S710$^*$& Ricoh GX100$^*$& Sony DSC-WX350\\ 
Apple iPhone 5& Canon Powershot ELPH 160& LG G3& Nikon D200$^*$& Rollei RCP-7325XS$^*$& Sony DSC-H50$^*$\\ 
Apple iPhone 5s& Canon Powershot S100& LG Nexus 5x& Nikon D3200& Samsung Galaxy Note4& Sony DSC-T77$^*$\\ 
Apple iPhone 6& Canon Powershot SX530 HS& Motorola Droid Maxx& Nikon D7100& Samsung Galaxy S2& Sony NEX-5TL\\ 
Apple iPhone 6+& Canon Powershot SX420 IS& Motorola Droid Turbo& Panasonic DMC-FZ50$^*$& Samsung Galaxy S4& \\ 
Apple iPhone 6s& Canon SX610 HS& Motorola X& Panasonic FZ200& Samsung L74wide$^*$& \\ 
Agfa Sensor530s$^*$& Casio EX-Z150$^*$& Motorola XT1060& Pentax K-7& Samsung NV15$^*$& \\ 
Canon EOS SL1& Fujifilm FinePix S8600& Nikon Coolpix S33& Pentax OptioA40$^*$& Sony DSC-H300& \\ 
\midrule
\multicolumn{6}{l}{\textbf{{Camera model set B}}} \\ 
Apple iPad Air 2& Canon Ixus70$^*$& Fujifilm FinePix XP80& LG Nexus 5& Olympus Stylus TG-860& Samsung Galaxy S3\\ 
Apple iPhone 5c& Canon PC1234& Fujifilm FinePix J50$^*$& Motorola Nexus 6& Panasonic TS30& Samsung Galaxy S5\\ 
Agfa DC-733s$^*$& Canon Powershot G10& HTC One M7& Nikon D70$^*$& Pentax OptioW60$^*$& Samsung Galaxy S7\\ 
Agfa DC-830i$^*$& Canon Powershot SX400 IS& Kodak EasyShare C813& Nikon D7000& Samsung Galaxy Note3& Sony A6000\\ 
Blackberry Leap& Canon T4i& Kodak M1063$^*$& Nokia Lumia 920& Samsung Galaxy Note5& Sony DSC-W170$^*$\\ 
\midrule
\multicolumn{6}{l}{\textbf{{Camera model set C}}} \\ 
Agfa DC-504$^*$& Canon Powershot A640$^*$& LG Realm& Olympus mju-1050SW$^*$& Samsung Galaxy Note2& \\ 
Agfa Sensor505x$^*$& Canon Rebel T3i& Nikon Coolpix S3700& Samsung Galaxy Lite& Samsung Galaxy S6 Edge& \\ 
Canon Ixus55$^*$& LG Optimus L90& Nikon D3000& Samsung Galaxy Nexus& Sony DSC-T70& \\ 
\midrule
\end{tabular}
\vspace{-4mm}
\end{table*}


==> tables/testfile_7.tex <==
\begin{table*}[t]\centering
\setlength{\tabcolsep}{0.5em}
\scriptsize
\begin{tabular}{l l l l l l l} 
\toprule
\multicolumn{7}{l}{\textbf{{Camera model set A}}} \\ 
Apple iPhone 4& Canon EOS SL1& Casio EX-Z150& Motorola X& Panasonic DMC-FZ50& Samsung Galaxy S2& Sony DSC-T77\\ 
Apple iPhone 4s& Canon PC1730& Fujifilm FinePix S8600& Motorola XT1060& Panasonic FZ200& Samsung Galaxy S4& Sony NEX-5TL\\ 
Apple iPhone 5& Canon Powershot A580& Huawei Honor 5x& Nikon Coolpix S33& Pentax K-7& Samsung L74wide& \\ 
Apple iPhone 5s& Canon Powershot ELPH 160& LG G2& Nikon Coolpix S7000& Pentax OptioA40& Samsung NV15& \\ 
Apple iPhone 6& Canon Powershot S100& LG G3& Nikon Coolpix S710& Praktica DCZ5.9& Sony DSC-H300& \\ 
Apple iPhone 6+& Canon Powershot SX530 HS& LG Nexus 5x& Nikon D200& Ricoh GX100& Sony DSC-W800& \\ 
Apple iPhone 6s& Canon Powershot SX420 IS& Motorola Droid Maxx& Nikon D3200& Rollei RCP-7325XS& Sony DSC-WX350& \\ 
Agfa Sensor530s& Canon SX610 HS& Motorola Droid Turbo& Nikon D7100& Samsung Galaxy Note4& Sony DSC-H50& \\ 
\midrule
\multicolumn{7}{l}{\textbf{{Camera model set B}}} \\ 
Apple iPad Air 2& Canon Ixus70& Fujifilm FinePix XP80& LG Nexus 5& Olympus Stylus TG-860& Samsung Galaxy S3& \\ 
Apple iPhone 5c& Canon PC1234& Fujifilm FinePix J50& Motorola Nexus 6& Panasonic TS30& Samsung Galaxy S5& \\ 
Agfa DC-733s& Canon Powershot G10& HTC One M7& Nikon D70& Pentax OptioW60& Samsung Galaxy S7& \\ 
Agfa DC-830i& Canon Powershot SX400 IS& Kodak EasyShare C813& Nikon D7000& Samsung Galaxy Note3& Sony A6000& \\ 
Blackberry Leap& Canon T4i& Kodak M1063& Nokia Lumia 920& Samsung Galaxy Note5& Sony DSC-W170& \\ 
\midrule
\multicolumn{7}{l}{\textbf{{Camera model set C}}} \\ 
Agfa DC-504& Canon PowershotA640& LG Realm& Olympus mju-1050SW& Samsung Galaxy Note2& & \\ 
Agfa Sensor505x& Canon Rebel T3i& Nikon Coolpix S3700& Samsung Galaxy Lite& Samsung Galaxy S6 Edge& & \\ 
Canon Ixus55& LG Optimus L90& Nikon D3000& Samsung Galaxy Nexus& Sony DSC-T70& & \\ 
\midrule
\end{tabular}
\end{table*}


==> tables/testfile_copy.tex <==
\begin{table*}\centering
\caption{Camera models used in training (sets A and B) and testing (set C). Note that $A\cap B =  A\cap C = B\cap C = 0$}
\label{tab:camera_models}
\begin{tabular}{l l l l} 
\toprule
\multicolumn{4}{l}{\textbf{{Camera model set A}}} \\ 
Apple iPhone 4& Canon PowerShot SX 530 HS& Nikon Coolpix S33& Samsung Galaxy Note4\\ 
Apple iPhone 4s& Canon PowerShot SX420 IS& Nikon Coolpix S7000& Samsung Galaxy S2\\ 
Apple iPhone 5& Canon SX610 HS& Nikon CoolPixS710& Samsung Galaxy S4\\ 
Apple iPhone 5s& Casio EX-Z150& Nikon D200& Samsung L74wide\\ 
Apple iPhone 6& Fujifilm FinePix S8600& Nikon D3200& Samsung NV15\\ 
Apple iPhone 6plus& Huawei Honor 5x& Nikon D7100& Sony CyberShot DSC-H300\\ 
Apple iPhone 6s& LG G2& Panasonic DMC-FZ50& Sony CyberShot DSC-W800\\ 
Agfa Sensor530s& LG G3& Panasonic FZ200& Sony Cybershot DSC-WX350\\ 
Canon EOS SL1& LG Nexus 5x& Pentax K-7& Sony DSC-H50\\ 
Canon PC1730& Motorola Droid Maxx& Pentax OptioA40& Sony DSC-T77\\ 
Canon PowerShot A580& Motorola Droid Turbo& Praktica DCZ5.9& Sony NEX-5TL\\ 
Canon PowerShot ELPH 160& Motorola X& Ricoh GX100& \\ 
Canon PowerShot S100& Motorola XT1060& Rollei RCP-7325XS& \\ 
\midrule
\multicolumn{4}{l}{\textbf{{Camera model set B}}} \\ 
Apple iPad Air 2& Canon PowerShot SX400 IS& Motorola Nexus 6& Samsung Galaxy Note5\\ 
Apple iPhone 5c& Canon T4i& Nikon D70& Samsung Galaxy S3\\ 
Agfa DC-733s& Fujifilm FinePix XP80& Nikon D7000& Samsung Galaxy S5\\ 
Agfa DC-830i& FujiFilm FinePixJ50& Nokia Lumia 920& Samsung Galaxy S7\\ 
Blackberry Leap& HTC One M7& Olympus Stylus Tough TG-860& Sony A6000\\ 
Canon Ixus70& Kodak EasyShare C813& Panasonic TS30& Sony DSC-W170\\ 
Canon PC1234& Kodak M1063& Pentax OptioW60& \\ 
Canon PowerShot G10& LG Nexus 5& Samsung Galaxy Note3& \\ 
\midrule
\multicolumn{4}{l}{\textbf{{Camera model set C}}} \\ 
Agfa DC-504& Canon Rebel T3i& Nikon D3000& Samsung Galaxy Note2\\ 
Agfa Sensor505-x& LG Optimus L90& Olympus mju-1050SW& Samsung Galaxy S6 Edge\\ 
Canon Ixus55& LG Realm& Samsung Galaxy Lite& Sony CyberShot DSC-T70\\ 
Canon PowerShotA640& Nikon Coolpix S3700& Samsung Galaxy Nexus& \\ 
\bottomrule
\end{tabular}
\end{table*}



==> tables/testfile_v1.tex <==
\begin{table*}[t]\centering
\caption{Camera models used in training (sets A and B) and testing (set C). Note that $A\cap B =  A\cap C = B\cap C = \emptyset$}
\label{tab:camera_models}
\begin{tabular}{l l l l l} 
\toprule
\multicolumn{5}{l}{\textbf{{Camera model set A}}} \\ 
Apple iPhone 4& Canon PowerShot A580& LG G3& Nikon D3200& Samsung Galaxy S2\\ 
Apple iPhone 4s& Canon PowerShot ELPH 160& LG Nexus 5x& Nikon D7100& Samsung Galaxy S4\\ 
Apple iPhone 5& Canon PowerShot S100& Motorola Droid Maxx& Panasonic DMC-FZ50& Samsung L74wide\\ 
Apple iPhone 5s& Canon PowerShot SX 530 HS& Motorola Droid Turbo& Panasonic FZ200& Samsung NV15\\ 
Apple iPhone 6& Canon PowerShot SX420 IS& Motorola X& Pentax K-7& Sony CyberShot DSC-H300\\ 
Apple iPhone 6plus& Canon SX610 HS& Motorola XT1060& Pentax OptioA40& Sony CyberShot DSC-W800\\ 
Apple iPhone 6s& Casio EX-Z150& Nikon Coolpix S33& Praktica DCZ5.9& Sony Cybershot DSC-WX350\\ 
Agfa Sensor530s& Fujifilm FinePix S8600& Nikon Coolpix S7000& Ricoh GX100& Sony DSC-H50\\ 
Canon EOS SL1& Huawei Honor 5x& Nikon CoolPixS710& Rollei RCP-7325XS& Sony DSC-T77\\ 
Canon PC1730& LG G2& Nikon D200& Samsung Galaxy Note4& Sony NEX-5TL\\ 
\midrule
\multicolumn{5}{l}{\textbf{{Camera model set B}}} \\ 
Apple iPad Air 2& Canon PC1234& HTC One M7& Nikon D7000& Samsung Galaxy Note5\\ 
Apple iPhone 5c& Canon PowerShot G10& Kodak EasyShare C813& Nokia Lumia 920& Samsung Galaxy S3\\ 
Agfa DC-733s& Canon PowerShot SX400 IS& Kodak M1063& Olympus Stylus Tough TG-860& Samsung Galaxy S5\\ 
Agfa DC-830i& Canon T4i& LG Nexus 5& Panasonic TS30& Samsung Galaxy S7\\ 
Blackberry Leap& Fujifilm FinePix XP80& Motorola Nexus 6& Pentax OptioW60& Sony A6000\\ 
Canon Ixus70& FujiFilm FinePixJ50& Nikon D70& Samsung Galaxy Note3& Sony DSC-W170\\ 
\midrule
\multicolumn{5}{l}{\textbf{{Camera model set C}}} \\ 
Agfa DC-504& Canon PowerShotA640& LG Realm& Olympus mju-1050SW& Samsung Galaxy Note2\\ 
Agfa Sensor505-x& Canon Rebel T3i& Nikon Coolpix S3700& Samsung Galaxy Lite& Samsung Galaxy S6 Edge\\ 
Canon Ixus55& LG Optimus L90& Nikon D3000& Samsung Galaxy Nexus& Sony CyberShot DSC-T70\\ 
\midrule
\end{tabular}
\end{table*}

